NeuralQA: A Usable Library for Question Answering (Contextual Query Expansion + BERT) on Large Datasets

Existing tools for Question Answering (QA) have challenges that limit their use in practice. They can be complex to set up or integrate with existing infrastructure, do not offer configurable interactive interfaces, and do not cover the full set of subtasks that frequently comprise the QA pipeline (query expansion, retrieval, reading, and explanation/sensemaking). To help address these issues, we introduce NeuralQA - a usable library for QA on large datasets. NeuralQA integrates well with existing infrastructure (e.g., ElasticSearch instances and reader models trained with the HuggingFace Transformers API) and offers helpful defaults for QA subtasks. It introduces and implements contextual query expansion (CQE) using a masked language model (MLM) as well as relevant snippets (RelSnip) - a method for condensing large documents into smaller passages that can be speedily processed by a document reader model. Finally, it offers a flexible user interface to support workflows for research explorations (e.g., visualization of gradient-based explanations to support qualitative inspection of model behaviour) and large scale search deployment. Code and documentation for NeuralQA is available as open source on Github (https://github.com/victordibia/neuralqa}{Github).

==> experiments.tex <==
\section{Experiments}

\input{experimentgraph}

We conducted several experiments and ablation studies  that inform the design choices implemented in NeuralQA.  Specifically, we explore the impact of passage fragmentation strategies, query expansion methods, retrieved passage concatenation \(RelSnip\) on QA performance. We define QA performance loosely as the \colorbox{yellow}{Andrew ..} ...

Our experiments are conducted using a subset of the Google natural questions dataset \colorbox{yellow}{ref}.

\input{experimenttable}

% [Andrew/Victor TODO] 
% - What subset of NQ was used?How was this subset extracted?
% - What are performance comparisons when we use different passage segmentation/fragmentaation strategies .. e.g. retrieve the whole passage from index vs break passage into paragraphs (or diff sizes) .. what is the run time cost for each of these?
% also, does smaller passages yield improved/more meaningful confidence signals?


% - What is performance (EM, F1, Runtime) when we leave the passage long, but construct a "relevant snippets" passage. Algo .. for a long passage (e.g. 5,000 tokens), 
%  i.) get a highlight snippet -  neighbourhood (e.g 150 characters) of top k text where each keyword match occurs. Elastic search supports this out of the box
%  ii.) concatenate each snippet to form a new "relevant snippet" passage of say 400 tokens
%  iii.) feed this 400 tokens to BERT instead of original 5,000 tokens. Much faster and practical !!!!
 
% - How does different query expansion methods impact performance (EM, F1, Runtime) ?  E.g PRM, Synonymns, RM3,  RM3+Word2Vec, RM3+Bert (this paper here seems to suggest this is a good idea but not always.. https://www.cs.cmu.edu/~zhuyund/papers/ECIR_2020.pdf),  query expansion token size (e.g. we add a maximum of 10, 15, 20 keywords to the initial query and review performance) 

% TODO: implement these things as standalone methods for neuralqa possibly based on spacy? A method that takes in a query, takes in an expansion method, + other kwargs and spits out an expanded query?
 
\subsection{Query Expansion}
\label{sec:queryexpansion}
We explore the following strategies for QE prior to document reading. 
i) BM25 Baseline ii.) Relevance Model \cite{lin2019neural} iii.) Finetuned Word2Vec Embeddings iv.) Finetuned MLM embeddings v.) 

\subsection{Passage Fragmentation with \(RelSnip\)}
\label{sec:relsnip} 
Findings from \cite{yang2019end} that a segmenting long documents into paragraphs prior to indexing provided better overall QA performance (almost 2x). We explore this option and also introduce a \textit{relevant snippet, \(RelSnip\)} approach that does not involve any custom indexing steps. A \(RelSnip\) is constructed as follows: For each long passage (e.g. 5,000 tokens) returned by BM25,  
 i.) get a highlight sections -  neighbourhood (e.g 150 characters) of top k text where each keyword match occurs. Elastic search supports this out of the box
 ii.) concatenate each snippet to form a new "relevant snippet" passage of say 400 tokens
 iii.) feed this 400 tokens to BERT based document reader instead of original 5,000 tokens. 
 In many practical cases, it may be challenging, redundant or undesirable to recreate indexes at the paragraph level. The \(RelSnip\) helps avoid that while also reducing the run time costs required for document reading. 
 
 
 adding some relevant papers to be read and processed 
 use search on mlm for query expansion 
 
 paper by ganguly et al and otsuka et al

==> experimenttable.tex <==

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{lllll}
% \hline
% Model & EM & F1 & \(IR_t\) & \(QA_t\) \\ \hline
% Baseline (BM25 + Bert) &  &  &  &  \\
% QE + RM3 &  &  &  &  \\
% QE + Word2Vec &  &  &  &  \\ \hline
% QE +  MLM &  &  &  &  \\ \hline
% CQE + MLM + RelSnip &  &  &  &  \\ \hline
% CQE + MLM + \(RelSnip\) (Par, k=218) &  &  &  &  \\ \hline
% \end{tabular}%
% }
% \caption{\label{tab:experimentresults} Results on NQ subset (questions with short answers) showing EM, F1 and runtime for the Information Retrieval and Docurment Reading parts of the task}
% \end{table}


% % \caption{\label{tab:experimentresults} Results on NQ subset (questions with short answers).}
% % \end{table}

==> overview.tex <==
\section{Overview}


 
